First Betti number of the path homology of random directed graphs

Path homology is a topological invariant for directed graphs, which is sensitive to their asymmetry and can discern between digraphs which are indistinguishable to the directed flag complex. In Erd\"os-R\'enyi directed random graphs, the first Betti number undergoes two distinct transitions, appearing at a low-density boundary and vanishing again at a high-density boundary. Through a novel, combinatorial condition for digraphs we describe both sparse and dense regimes under which the first Betti number of path homology is zero with high probability. We combine results of Grigor'yan et al., regarding generators for chain groups, with methods of Kahle and Meckes in order to determine regimes under which the first Betti number is positive with high probability. Together, these results describe the gradient of the lower boundary and yield bounds for the gradient of the upper boundary. With a view towards hypothesis testing, we obtain tighter bounds on the probability of observing a positive first Betti number in a high-density digraph of finite size. For comparison, we apply these techniques to the directed flag complex and derive analogous results.

==> sections/applications.tex <==
\section{Applications}
\label{sec:apply}
\subsection{E-mail networks}
Now that we have a better understanding of the behaviour of path homology on random graphs we can investigate practical applications.
We study the \texttt{email-Eu-core} directed graph dataset from SNAP \cite{snapnets} -- a directed graph of email correspondence between members of a European research institution.
The graph includes a directed edge $(i,j)$ if individual $i$ sent individual $j$ at least one email.
Nodes of the network are labelled according to the correspondent's home department, providing a partition into 42 canonical communities.
Note, \citeauthor{Chowdhury2020} used path homology to analyse a temporal version of this dataset in \cite{Chowdhury2020}.
To investigate the network, we consider the subnetwork $G_c$ of each community $c$.
For each such community we sample 4199 random directed graphs $\dir{G}(n,p)$ where $n = \abs{V(G_c)}$ and $p= \abs{E(G_c)}/(n(n-1))$.
For the sampled graphs and community graph we compute $\betti_1$, in order to execute a Monte Carlo test.
The computed $\betti_1$ are ordered and, when $p$ is outside or near to the conjectured boundaries, we consider a large value of $\betti_1$ to be significant.
To counteract the problem of multiple comparisons we use Bonferroni correction.
To obtain a significance level of $\alpha = 5/100$, $\betti_1$ of the community digraph must lie within the first 5 of the ordered Betti numbers.
We obtain statistically significant results only in departments 1 and 4, which are the third and first largest departments respectively.
In comparison, departments 1,4,6,15,23,29 and 30 all of non-trivial $\betti_1$.
This statistical approach helps to highlight graphs with interesting structure, i.e. structure that we would not predict based purely on graph density.


